Demonstration of new MeV-scale capabilities in large neutrino LArTPCs using ambient radiogenic and cosmogenic activity in MicroBooNE

Large neutrino liquid argon time projection chamber (LArTPC) experiments can broaden their physics reach by reconstructing and interpreting MeV-scale energy depositions, or blips, present in their data. We demonstrate new calorimetric and particle discrimination capabilities at the MeV energy scale using reconstructed blips in data from the MicroBooNE LArTPC at Fermilab. We observe a concentration of low energy ($<$3~MeV) blips around fiberglass mechanical support struts along the TPC edges with energy spectrum features consistent with the Compton edge of 2.614 MeV $^{208}$Tl decay $\gamma$~rays. These features are used to verify proper calibration of electron energy scales in MicroBooNE's data to few percent precision and to measure the specific activity of $^{208}$Tl in the fiberglass composing these struts, $(11.7 \pm 0.2 ~\text{(stat)} \pm 3.1~\text{(syst)})$~Bq/kg. Cosmogenically-produced blips above 3~MeV in reconstructed energy are used to showcase the ability of large LArTPCs to distinguish between low-energy proton and electron energy depositions. An enriched sample of low-energy protons selected using this new particle discrimination technique is found to be smaller in data than in dedicated CORSIKA cosmic ray simulations, suggesting either incorrect CORSIKA modeling of incident cosmic fluxes or particle transport modeling issues in Geant4.

==> authors.tex <==
%####### AUTHORS ######
% List of institutions in command form:
%MicroBooNE_AuthorList_July2024
\newcommand{\ANL}{Argonne National Laboratory (ANL), Lemont, IL, 60439, USA}
\newcommand{\Bern}{Universit{\"a}t Bern, Bern CH-3012, Switzerland}
\newcommand{\BNL}{Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}
\newcommand{\UCSB}{University of California, Santa Barbara, CA, 93106, USA}
\newcommand{\Cambridge}{University of Cambridge, Cambridge CB3 0HE, United Kingdom}
\newcommand{\CIEMAT}{Centro de Investigaciones Energ\'{e}ticas, Medioambientales y Tecnol\'{o}gicas (CIEMAT), Madrid E-28040, Spain}
\newcommand{\Chicago}{University of Chicago, Chicago, IL, 60637, USA}
\newcommand{\Cincinnati}{University of Cincinnati, Cincinnati, OH, 45221, USA}
\newcommand{\CSU}{Colorado State University, Fort Collins, CO, 80523, USA}
\newcommand{\Columbia}{Columbia University, New York, NY, 10027, USA}
\newcommand{\Edinburgh}{University of Edinburgh, Edinburgh EH9 3FD, United Kingdom}
\newcommand{\FNAL}{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}
\newcommand{\Granada}{Universidad de Granada, Granada E-18071, Spain}
\newcommand{\IIT}{Illinois Institute of Technology (IIT), Chicago, IL 60616, USA}
\newcommand{\ICL}{Imperial College London, London SW7 2AZ, United Kingdom}
\newcommand{\Indiana}{Indiana University, Bloomington, IN 47405, USA}
\newcommand{\KSU}{Kansas State University (KSU), Manhattan, KS, 66506, USA}
\newcommand{\Lancaster}{Lancaster University, Lancaster LA1 4YW, United Kingdom}
\newcommand{\LANL}{Los Alamos National Laboratory (LANL), Los Alamos, NM, 87545, USA}
\newcommand{\Louisiana}{Louisiana State University, Baton Rouge, LA, 70803, USA}
\newcommand{\Manchester}{The University of Manchester, Manchester M13 9PL, United Kingdom}
\newcommand{\MIT}{Massachusetts Institute of Technology (MIT), Cambridge, MA, 02139, USA}
\newcommand{\Michigan}{University of Michigan, Ann Arbor, MI, 48109, USA}
\newcommand{\MSU}{Michigan State University, East Lansing, MI 48824, USA}
\newcommand{\Minnesota}{University of Minnesota, Minneapolis, MN, 55455, USA}
\newcommand{\Nankai}{Nankai University, Nankai District, Tianjin 300071, China}
\newcommand{\NMSU}{New Mexico State University (NMSU), Las Cruces, NM, 88003, USA}
\newcommand{\Oxford}{University of Oxford, Oxford OX1 3RH, United Kingdom}
\newcommand{\Pitt}{University of Pittsburgh, Pittsburgh, PA, 15260, USA}
\newcommand{\QMUL}{Queen Mary University of London, London E1 4NS, United Kingdom}
\newcommand{\Rutgers}{Rutgers University, Piscataway, NJ, 08854, USA}
\newcommand{\SLAC}{SLAC National Accelerator Laboratory, Menlo Park, CA, 94025, USA}
\newcommand{\SDSMT}{South Dakota School of Mines and Technology (SDSMT), Rapid City, SD, 57701, USA}
\newcommand{\Maine}{University of Southern Maine, Portland, ME, 04104, USA}
\newcommand{\Syracuse}{Syracuse University, Syracuse, NY, 13244, USA}
\newcommand{\TelAviv}{Tel Aviv University, Tel Aviv, Israel, 69978}
\newcommand{\UTA}{University of Texas, Arlington, TX, 76019, USA}
\newcommand{\Tufts}{Tufts University, Medford, MA, 02155, USA}
\newcommand{\VTech}{Center for Neutrino Physics, Virginia Tech, Blacksburg, VA, 24061, USA}
\newcommand{\Warwick}{University of Warwick, Coventry CV4 7AL, United Kingdom}


% So that institutions appear in alphabetical order:
\affiliation{\ANL}
\affiliation{\Bern}
\affiliation{\BNL}
\affiliation{\UCSB}
\affiliation{\Cambridge}
\affiliation{\CIEMAT}
\affiliation{\Chicago}
\affiliation{\Cincinnati}
\affiliation{\CSU}
\affiliation{\Columbia}
\affiliation{\Edinburgh}
\affiliation{\FNAL}
\affiliation{\Granada}
\affiliation{\IIT}
\affiliation{\ICL}
\affiliation{\Indiana}
\affiliation{\KSU}
\affiliation{\Lancaster}
\affiliation{\LANL}
\affiliation{\Louisiana}
\affiliation{\Manchester}
\affiliation{\MIT}
\affiliation{\Michigan}
\affiliation{\MSU}
\affiliation{\Minnesota}
\affiliation{\Nankai}
\affiliation{\NMSU}
\affiliation{\Oxford}
\affiliation{\Pitt}
\affiliation{\QMUL}
\affiliation{\Rutgers}
\affiliation{\SLAC}
\affiliation{\SDSMT}
\affiliation{\Maine}
\affiliation{\Syracuse}
\affiliation{\TelAviv}
\affiliation{\UTA}
\affiliation{\Tufts}
\affiliation{\VTech}
\affiliation{\Warwick}

% Authors in alphabetical order
\author{P.~Abratenko} \affiliation{\Tufts}
\author{O.~Alterkait} \affiliation{\Tufts}
\author{D.~Andrade~Aldana} \affiliation{\IIT}
\author{L.~Arellano} \affiliation{\Manchester}
\author{J.~Asaadi} \affiliation{\UTA}
\author{A.~Ashkenazi}\affiliation{\TelAviv}
\author{S.~Balasubramanian}\affiliation{\FNAL}
\author{B.~Baller} \affiliation{\FNAL}
\author{A.~Barnard} \affiliation{\Oxford}
\author{G.~Barr} \affiliation{\Oxford}
\author{D.~Barrow} \affiliation{\Oxford}
\author{J.~Barrow} \affiliation{\Minnesota}
\author{V.~Basque} \affiliation{\FNAL}
\author{J.~Bateman} \affiliation{\Manchester}
\author{O.~Benevides~Rodrigues} \affiliation{\IIT}
\author{S.~Berkman} \affiliation{\MSU}
\author{A.~Bhanderi} \affiliation{\Manchester}
\author{A.~Bhat} \affiliation{\Chicago}
\author{M.~Bhattacharya} \affiliation{\FNAL}
\author{M.~Bishai} \affiliation{\BNL}
\author{A.~Blake} \affiliation{\Lancaster}
\author{B.~Bogart} \affiliation{\Michigan}
\author{T.~Bolton} \affiliation{\KSU}
\author{M.~B.~Brunetti} \affiliation{\Warwick}
\author{L.~Camilleri} \affiliation{\Columbia}
\author{Y.~Cao} \affiliation{\Manchester}
\author{D.~Caratelli} \affiliation{\UCSB}
\author{F.~Cavanna} \affiliation{\FNAL}
\author{G.~Cerati} \affiliation{\FNAL}
\author{A.~Chappell} \affiliation{\Warwick}
\author{Y.~Chen} \affiliation{\SLAC}
\author{J.~M.~Conrad} \affiliation{\MIT}
\author{M.~Convery} \affiliation{\SLAC}
\author{L.~Cooper-Troendle} \affiliation{\Pitt}
\author{J.~I.~Crespo-Anad\'{o}n} \affiliation{\CIEMAT}
\author{R.~Cross} \affiliation{\Warwick}
\author{M.~Del~Tutto} \affiliation{\FNAL}
\author{S.~R.~Dennis} \affiliation{\Cambridge}
\author{P.~Detje} \affiliation{\Cambridge}
\author{R.~Diurba} \affiliation{\Bern}
\author{Z.~Djurcic} \affiliation{\ANL}
\author{K.~Duffy} \affiliation{\Oxford}
\author{S.~Dytman} \affiliation{\Pitt}
\author{B.~Eberly} \affiliation{\Maine}
\author{P.~Englezos} \affiliation{\Rutgers}
\author{A.~Ereditato} \affiliation{\Chicago}\affiliation{\FNAL}
\author{J.~J.~Evans} \affiliation{\Manchester}
\author{C.~Fang} \affiliation{\UCSB}
\author{W.~Foreman} \affiliation{\IIT} \affiliation{\LANL}
\author{B.~T.~Fleming} \affiliation{\Chicago}
\author{D.~Franco} \affiliation{\Chicago}
\author{A.~P.~Furmanski}\affiliation{\Minnesota}
\author{F.~Gao}\affiliation{\UCSB}
\author{D.~Garcia-Gamez} \affiliation{\Granada}
\author{S.~Gardiner} \affiliation{\FNAL}
\author{G.~Ge} \affiliation{\Columbia}
\author{S.~Gollapinni} \affiliation{\LANL}
\author{E.~Gramellini} \affiliation{\Manchester}
\author{P.~Green} \affiliation{\Oxford}
\author{H.~Greenlee} \affiliation{\FNAL}
\author{L.~Gu} \affiliation{\Lancaster}
\author{W.~Gu} \affiliation{\BNL}
\author{R.~Guenette} \affiliation{\Manchester}
\author{P.~Guzowski} \affiliation{\Manchester}
\author{L.~Hagaman} \affiliation{\Chicago}
\author{M.~D.~Handley} \affiliation{\Cambridge}
\author{O.~Hen} \affiliation{\MIT}
\author{C.~Hilgenberg}\affiliation{\Minnesota}
\author{G.~A.~Horton-Smith} \affiliation{\KSU}
\author{Z.~Imani} \affiliation{\Tufts}
\author{B.~Irwin} \affiliation{\Minnesota}
\author{M.~S.~Ismail} \affiliation{\Pitt}
\author{C.~James} \affiliation{\FNAL}
\author{X.~Ji} \affiliation{\Nankai}
\author{J.~H.~Jo} \affiliation{\BNL}
\author{R.~A.~Johnson} \affiliation{\Cincinnati}
\author{Y.-J.~Jwa} \affiliation{\Columbia}
\author{D.~Kalra} \affiliation{\Columbia}
\author{G.~Karagiorgi} \affiliation{\Columbia}
\author{W.~Ketchum} \affiliation{\FNAL}
\author{M.~Kirby} \affiliation{\BNL}
\author{T.~Kobilarcik} \affiliation{\FNAL}
\author{N.~Lane} \affiliation{\Manchester}
\author{J.-Y. Li} \affiliation{\Edinburgh}
\author{Y.~Li} \affiliation{\BNL}
\author{K.~Lin} \affiliation{\Rutgers}
\author{B.~R.~Littlejohn} \affiliation{\IIT}
\author{L.~Liu} \affiliation{\FNAL}
\author{W.~C.~Louis} \affiliation{\LANL}
\author{X.~Luo} \affiliation{\UCSB}
\author{T.~Mahmud} \affiliation{\Lancaster}
\author{C.~Mariani} \affiliation{\VTech}
\author{D.~Marsden} \affiliation{\Manchester}
\author{J.~Marshall} \affiliation{\Warwick}
\author{N.~Martinez} \affiliation{\KSU}
\author{D.~A.~Martinez~Caicedo} \affiliation{\SDSMT}
\author{S.~Martynenko} \affiliation{\BNL}
\author{A.~Mastbaum} \affiliation{\Rutgers}
\author{I.~Mawby} \affiliation{\Lancaster}
\author{N.~McConkey} \affiliation{\QMUL}
\author{V.~Meddage} \affiliation{\KSU}
\author{L.~Mellet} \affiliation{\MSU}
\author{J.~Mendez} \affiliation{\Louisiana}
\author{J.~Micallef} \affiliation{\MIT}\affiliation{\Tufts}
\author{K.~Miller} \affiliation{\Chicago}
\author{A.~Mogan} \affiliation{\CSU}
\author{T.~Mohayai} \affiliation{\Indiana}
\author{M.~Mooney} \affiliation{\CSU}
\author{A.~F.~Moor} \affiliation{\Cambridge}
\author{C.~D.~Moore} \affiliation{\FNAL}
\author{L.~Mora~Lepin} \affiliation{\Manchester}
\author{M.~M.~Moudgalya} \affiliation{\Manchester}
\author{S.~Mulleriababu} \affiliation{\Bern}
\author{D.~Naples} \affiliation{\Pitt}
\author{A.~Navrer-Agasson} \affiliation{\ICL} \affiliation{\Manchester}
\author{N.~Nayak} \affiliation{\BNL}
\author{M.~Nebot-Guinot}\affiliation{\Edinburgh}
\author{C.~Nguyen}\affiliation{\Rutgers}
\author{J.~Nowak} \affiliation{\Lancaster}
\author{N.~Oza} \affiliation{\Columbia}
\author{O.~Palamara} \affiliation{\FNAL}
\author{N.~Pallat} \affiliation{\Minnesota}
\author{V.~Paolone} \affiliation{\Pitt}
\author{A.~Papadopoulou} \affiliation{\ANL}
\author{V.~Papavassiliou} \affiliation{\NMSU}
\author{H.~B.~Parkinson} \affiliation{\Edinburgh}
\author{S.~F.~Pate} \affiliation{\NMSU}
\author{N.~Patel} \affiliation{\Lancaster}
\author{Z.~Pavlovic} \affiliation{\FNAL}
\author{E.~Piasetzky} \affiliation{\TelAviv}
\author{K.~Pletcher} \affiliation{\MSU}
\author{I.~Pophale} \affiliation{\Lancaster}
\author{X.~Qian} \affiliation{\BNL}
\author{J.~L.~Raaf} \affiliation{\FNAL}
\author{V.~Radeka} \affiliation{\BNL}
\author{A.~Rafique} \affiliation{\ANL}
\author{M.~Reggiani-Guzzo} \affiliation{\Edinburgh}
\author{L.~Ren} \affiliation{\NMSU}
\author{L.~Rochester} \affiliation{\SLAC}
\author{J.~Rodriguez Rondon} \affiliation{\SDSMT}
\author{M.~Rosenberg} \affiliation{\Tufts}
\author{M.~Ross-Lonergan} \affiliation{\LANL}
\author{I.~Safa} \affiliation{\Columbia}
\author{D.~W.~Schmitz} \affiliation{\Chicago}
\author{A.~Schukraft} \affiliation{\FNAL}
\author{W.~Seligman} \affiliation{\Columbia}
\author{M.~H.~Shaevitz} \affiliation{\Columbia}
\author{R.~Sharankova} \affiliation{\FNAL}
\author{J.~Shi} \affiliation{\Cambridge}
\author{E.~L.~Snider} \affiliation{\FNAL}
\author{M.~Soderberg} \affiliation{\Syracuse}
\author{S.~S{\"o}ldner-Rembold} \affiliation{\ICL} \affiliation{\Manchester}
\author{J.~Spitz} \affiliation{\Michigan}
\author{M.~Stancari} \affiliation{\FNAL}
\author{J.~St.~John} \affiliation{\FNAL}
\author{T.~Strauss} \affiliation{\FNAL}
\author{A.~M.~Szelc} \affiliation{\Edinburgh}
\author{N.~Taniuchi} \affiliation{\Cambridge}
\author{K.~Terao} \affiliation{\SLAC}
\author{C.~Thorpe} \affiliation{\Manchester}
\author{D.~Torbunov} \affiliation{\BNL}
\author{D.~Totani} \affiliation{\UCSB}
\author{M.~Toups} \affiliation{\FNAL}
\author{A.~Trettin} \affiliation{\Manchester}
\author{Y.-T.~Tsai} \affiliation{\SLAC}
\author{J.~Tyler} \affiliation{\KSU}
\author{M.~A.~Uchida} \affiliation{\Cambridge}
\author{T.~Usher} \affiliation{\SLAC}
\author{B.~Viren} \affiliation{\BNL}
\author{J.~Wang} \affiliation{\Nankai}
\author{M.~Weber} \affiliation{\Bern}
\author{H.~Wei} \affiliation{\Louisiana}
\author{A.~J.~White} \affiliation{\Chicago}
\author{S.~Wolbers} \affiliation{\FNAL}
\author{T.~Wongjirad} \affiliation{\Tufts}
\author{M.~Wospakrik} \affiliation{\FNAL}
\author{K.~Wresilo} \affiliation{\Cambridge}
\author{W.~Wu} \affiliation{\Pitt}
\author{E.~Yandel} \affiliation{\UCSB} \affiliation{\LANL} 
\author{T.~Yang} \affiliation{\FNAL}
\author{L.~E.~Yates} \affiliation{\FNAL}
\author{H.~W.~Yu} \affiliation{\BNL}
\author{G.~P.~Zeller} \affiliation{\FNAL}
\author{J.~Zennamo} \affiliation{\FNAL}
\author{C.~Zhang} \affiliation{\BNL}

\collaboration{The MicroBooNE Collaboration}
\thanks{microboone\_info@fnal.gov}\noaffiliation

